Human Response to an AI-Based Decision Support System: A User Study on the Effects of Accuracy and Bias

Artificial Intelligence (AI) is increasingly used to build Decision Support Systems (DSS) across many domains. This paper describes a series of experiments designed to observe human response to different characteristics of a DSS such as accuracy and bias, particularly the extent to which participants rely on the DSS, and the performance they achieve. In our experiments, participants play a simple online game inspired by so-called "wildcat" (i.e., exploratory) drilling for oil. The landscape has two layers: a visible layer describing the costs (terrain), and a hidden layer describing the reward (oil yield). Participants in the control group play the game without receiving any assistance, while in treatment groups they are assisted by a DSS suggesting places to drill. For certain treatments, the DSS does not consider costs, but only rewards, which introduces a bias that is observable by users. Between subjects, we vary the accuracy and bias of the DSS, and observe the participants' total score, time to completion, the extent to which they follow or ignore suggestions. We also measure the acceptability of the DSS in an exit survey. Our results show that participants tend to score better with the DSS, that the score increase is due to users following the DSS advice, and related to the difficulty of the game and the accuracy of the DSS. We observe that this setting elicits mostly rational behavior from participants, who place a moderate amount of trust in the DSS and show neither algorithmic aversion (under-reliance) nor automation bias (over-reliance).However, their stated willingness to accept the DSS in the exit survey seems less sensitive to the accuracy of the DSS than their behavior, suggesting that users are only partially aware of the (lack of) accuracy of the DSS.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> Sections/99.Removed.tex <==

\clearpage
\section{Removed from the introduction}

For instance, multiple research efforts use advanced machine learning and deep learning imaging-based techniques to assist physicians overcome the challenge of early tumor detection \cite{lotlikar_2021}.
\mynote[from=Manuel]{As a starting example I would put something closer to the case, because image analysis is far from what is proposed in the experiment. It could be something related to automated decision-making systems used in government or something related with geotecnologies (given that the experiment is kind of a map).}
\mynote[from=ChaTo]{Agree}


Such domains are particularly interesting due to the negative implications incorrect decisions might have. 
\mynote[from=ChaTo]{I wouldn't mention high-stakes scenarios as our game is intentionally low-stakes}

\section{Removed Definition of Lucker}

Players were categorized between the following three types:
\begin{inparaenum}[(i)]
    \item lucker,
    \item learner and
    \item non-optimal explorer.
\end{inparaenum}
%
Corresponding respectivelly to those players that found a very good spot at the very begining of the game, those who improved during the game and those who did not improve the obtained score during their plays.
%
We analyzed the playing traces to select the two maps that have lower rates of lucker players and to them, we added a third map that was randomly selected between the maps with higher average score.

\section{Removed Perceived Map Difficulty}

After playing the three games, the users are asked to answer a short survey asking them for the map that was perceived as more easy.
%
Figure~\ref{fig:perceived_map_difficulty} shows the obtained results, where Map 2 was identified as the easier one and Map 5 the most difficult.
%
Results are aligned with the average score obtained in each map.


\begin{figure}[ht] % picture
    \centering
    \includegraphics[width=0.3\textwidth]{Figures/no_DSS_perceived_map_difficulty.png}
    \caption{Easiest map survey results.}
    \label{fig:perceived_map_difficulty}
\end{figure}

\section{RemovedAcceptance and Forest Cost}

\begin{figure}[ht] % picture
    \centering
    \includegraphics[width=0.35\textwidth]{Figures/TAM_forest_cost.png}
    \caption{Technology acceptance survey results by forest cost. }
    \label{fig:TAM_survey_forest_cost}
\end{figure}

After, we assess the answers given to the technology acceptance survey depending on the cost of the forest cells.
%
We have reduced the number of bins in the histogram to reduce noise.
%
With that, we observe that the machine assistance is slightly better valued when the cost is higher.
%

\section{Removed Acceptance and Model bias}

\begin{figure}[ht] % picture
    \centering
    \includegraphics[width=0.35\textwidth]{Figures/TAM_cost_awareness.png}
    \caption{Technology acceptance survey results by model bias. }
    \label{fig:TAM_survey_model_bias}
\end{figure}

After, we assess the answers given to the technology acceptance survey depending on the cost of the forest cells.
%
We have reduced the number of bins in the histogram to reduce noise.
%
With that, we observe that the machine assistance is slightly better valued when the cost is higher.
%

\section{Removed from learning effects}

We also compared the distributions of socio-demographic between the obtained communities. No statistically significant differences were found.


==> Sections_OLD/0.Abstract.tex <==
This research project is focused on the study of human interaction with automatic systems designed to assist users during decision making processes. In particular, we present a platform that allows researchers to quantify the extent up to which individuals change or adapt their behaviour depending on different characteristics of the automatic system in a controlled environment.
\mynote[from=Manuel]{If the focus is the platform and not only the study we should give more importance to it and being more specific (> automatic systems) }

To conduct the experiments, a decision support system (DSS) can be added to help users to complete their tasks.
The developed experimental platform allows researchers to control different characteristics of the DSS and the environment such as the predictive accuracy of the system, the presence or not of biased predictions or the cost/income ratios of each zone of the map.


The objective then is to determine how them affect the human perception and therefore, the manner how individuals interact with the environment and it includes a set of surveys to understand the user perception of the system capacities.
To quantify it from the user participation, the platform is prepared to collect data such as the obtained score, the time to answer or the positions that where clicked between other things.

Capacities of the platform as well as the quality of the data that is produced by participants have been validated through different studies carried out using a crowdsourcing platform to recruit participants, collecting data from more than 400 users. 

Our results show, between other things, that users tend to increase their performance in terms of obtained score with the presence of an algorihtmic-based DSS and it occurs even when the DSS has los \textcolor{blue}{is this loss or lost?} accuracy. Additionally, they require more time to complete a game when there is a DSS, what can be an indicator of more time invested in decision-making.


We challenge other researchers to conduct new experiments with independent variables that lead to a behaviours that are different from what has been observed in this first round of experiments.

==> Sections_OLD/0.Abstract_OLD.tex <==

This research project is focused on the study of human interaction with automatic systems designed to assist users during decision making processes. In particular, the experiments study how individuals change or adapt their behaviour depending on different characteristics of the automatic system. 

During its execution, we aim to perform an empirical study to determine how (i) different levels of accuracy, (ii) the presence of biased predictions affect the human perception and therefore, the manner how individuals interact with the environment.

In this paper, we conduct a comparative user study on the effects of using an algorithm-based decision support system to help user solving their goal in a complex environment. 
The task users aim to solve is to maximize the score they get in an online game with twenty-five rounds where, in order to achieve their goal, users need to correctly balance exploration/exploitation to find and properly exploit the area where the global maximum is located.

The experimental setup consists in an online game with a 32x32 board composed by two layers. The first layer remains visible to the user and is formed by the terrain, composed by desert and forest cells. The second layer contains the oil, what corresponds to the income the user can get in each cell, the oil is hidden to the user until they click a cell, what reveals its content. The oil of each two neighbor cells is similar and the cost of drilling the forest is higher than drilling in the dessert. The values contained in both the terrain and forest layers are not correlated between them.

The set of dependent variables considered includes the total obtained score, the required amount of time to complete a game and the distance from the DSS suggestions to the clicked cells.

To conduct the study, we use a crowdsourcing platform to recruit participants, obtaining results with more than 400 users. 

Our results show, between other things, that users tend to increase their performance in terms of obtained score with the presence of an algorihtmic-based DSS. Additionally, they require more time to complete a game when there is a DSS, what can be an indicator of more time invested in decision-making.




Additional Key Words and Phrases: human-in-the-loop, human oversight

==> Sections_OLD/1.Introduction.tex <==
\section{Introduction}

Use cases where users are required to make decisions based or assisted on algorithmic-based recommendations are becoming more and more common in several domains.
%
For instance, several research efforts use advanced machine learning and deep learning imaging-based techniques to assist physicians overcome the challenge of early tumor detection \cite{lotlikar_2021}. 
%
Such domains are particularly interesting due to the negative implications incorrect decisions might have. 


Even if we assume automated systems are able to provide perfect predictions, still it is the human who is in charge or taking the final decision based on the inputs they have. 
%
The process of accounting for the machine predictions becomes way more complex when we consider that machines are still far from achieving perfect accuracy in such domains.


Several authors have studied and tested several techniques to increase user trust in the machine predictions \cite{Balfe2018UnderstandingIK}.
%
Nevertheless, we claim here that blindly incrementing trust on the machine predictions might not be the ideal case. \inote{why? -M}
%
Instead, \textbf{we aim to understand what are the conditions under which users are able to trust the predictions when they are correct and still have the tools so that the user is able to distrust the cases when the predictions are not so good}.
%
In particular, we are interested on the role of biased predictions \inote{where?} and to what extent the fact that the system is not giving predictions that are equally good between for all cases affects the user behaviour. 

\mynote[from=Manuel]{As a reader, just now I understand that we are talking about a game and not another kind of ADMS/DSS}
In this context, we developed a platform that allows researchers to conduct experiments under different conditions in a controlled environment. 
%
The proposed environment consists in an online game with a 32x32 map board composed by two layers. The first layer remains visible to the user and is formed by the terrain, composed by desert and forest cells. 
%
The second layer contains the oil, what corresponds to the income the user can get in each cell, the oil is hidden to the user until they click a cell, what reveals its content. 
%
The oil of each two neighbor cells is similar and the cost of drilling the forest is higher than drilling in the dessert. The values contained in both the terrain and forest layers are not correlated between them.


In such environment, researchers might first want to design a collection of boards to be used for experimentation. 
%
After, such maps can be used to understand what is the behaviour of experiment participants when there is no machine-based assistance or decision support system (DSS).


To incorporate a DSS, researchers can evaluate user performance where the DSS consideres only the income (so the predictive error is higher for forest cells where the cost is higher). \mynote[from=Manuel]{This is the argument of why is important the proposed system, maybe before explain it, add this as a motivation}
%
Additionally, there is the option of assessing the case where the system takes into consideration both income and cost, so the predictive error is evenly distributed across all cell types.



Two hypothesis guide our work:
\begin{itemize}
    \item{H1: Users are more open to take risks when they detect that the system predictions have good quality}
    \item{H2: Using a DSS, regardless of its real quality\inote{maybe performance? what is "real"?}, reduces the chances of very bad games while also reducing the exploration time}
\end{itemize}




==> Sections_OLD/2.RelatedWork.tex <==
\section{Related work}

\subsection{Decision making under assistance}
\mynote[from=Manuel]{From both papers below, maybe this is going too back in time and taking much space. Are these theories going to be discussed or are just framing the experiment?}
\textcolor{blue}{In their classic paper, authors of \cite{Tversky1974JudgmentUU} described three heuristics that are employed by humans in making judgments under uncertainty: (i) \textit{representativeness}, which is usually employed when people are asked to judge the probability that an object or event A belongs to class or process B; (ii) \textit{availability of instances or scenarios}, which is often employed when people are asked to assess the frequency of a class or the plausibility of a particular development; and (iii) \textit{adjustment from an anchor}, which is usually employed in numerical prediction when a relevant value is available. These heuristics are highly economical and usually effective, but they lead to systematic and predictable errors. A better understanding of these heuristics and of the biases to which they lead could improve judgments and decisions in situations of uncertainty.}

Also, authors of \cite{Arkes_1986} related how overconfidence can negatively affect the final performance since overconfident individuals tend to feel that no assistance
is needed. In their experiments, they observed that the more
knowledgeable subjects were less likely to use the proposed decision rules, which resulted
in inferior performance. 

In their more recent work, authors of \cite{Kleinberg_2017} described, in the criminal-justice context, the framework used here as: $$Data \rightarrow Prediction \rightarrow Decision$$ and describe the role of the algorithms as strictly focused in the first link (calculating predictions over the observed data) whereas the second link remains unconsidered for the automatic system. Also, in their work, they pointed to the importance of having a better knowledge of this second link to improve performance of the final decisions made in relation with machine predictions. \mynote[from=Manuel]{I was thinking that we should refer to other kinds of DSS, for example those used in urban or rural development, or something related to these tradeoffs more related, because decisions in justice is very far away from the game's idea. I will look for references.}


\subsection{Trust on automation}
\mynote[from=Manuel]{Is trust what you want to accomplish? I'm from the idea that is better to avoid such discussion because is too complex to address in an article that is more technical. Maybe convincing audience that this tool will help to address trust could be too much to ask.Because trust is contextual and situated, it is difficult to extrapolate findings to other domains.}
Literature on Trust on automation \cite{Balfe2018UnderstandingIK} defines the process of building trust as a three-stages model, driven by a first phase that requires the creation of a good mental model of the system behaviour, implying a certain necessity of understanding how the system works and therefore, some level of \textit{explainability}. After, the second stage is related to the capacity of the system of working as expected, which is related with \textit{reliability}, \textit{competence} and \textit{robustness}. Finally, the last stage is related to \textit{faith}, and has special interest in those cases where the capacities of the system exceed the operator's competence. The operator is therefore unable to evaluate the automation and must rely on an assessment of the automation’s responsibility.

\textcolor{blue}{Several researchers have
examined the factors influencing trust, and these
are summarized in two studies (Hoff and Bashir,2015; Schaefer et al., 2014). Both suggest that
trust is influenced by three sources: The first is
related to the individual, including his or her
personality, background, attitudes, and capabilities, and can be labeled dispositional trust. The 
second relates to the situation or environment,
including the complexity of the task and the
operator workload, and can be labeled situational trust. The third relates to the automation
itself, including its behavior, reliability, transparency, and performance, and can be labeled
learned trust.}

The work done by \citet{Balfe2018UnderstandingIK} shows that previous literature on Trust on Automation has detected the following attributes as highly relevant items to the process of explaining what drives trust on the automated system:

\begin{enumerate}
\item{ \textbf{reliability}—in terms of both mechanical reliability and consistent functioning over time (Madsen
\& Gregor, 2000; Muir \& Moray, 1996; Sheridan,
1999);}
\item{ \textbf{robustness}—the ability to function under a variety
of circumstances (Sheridan, 1999; Woods, 1996);}
\item{ \textbf{understandability}—the ability to understand what
the automation is doing, why it is doing it, and
how it is doing it (Madsen \& Gregor, 2000; Sheridan, 1999);}
\item{ \textbf{competence}—the perceived ability of the automation to perform its tasks (Madsen \& Gregor, 2000;
Muir \& Moray, 1996)}
\item{ \textbf{feedback}—the ability of the automation to explicitly give feedback on its intended actions (Norman, 1990; Sheridan, 1999)}
\item{ \textbf{dependability}—the extent to which the automation can be counted on to do its job (Muir \&
Moray, 1996; Rempel et al., 1985)}
\item{ \textbf{personal attachment}—the extent to which operators like to use the automation (Madsen \& Gregor,
2000)}
\item{ \textbf{predictability}—the ability of the operator to predict the actions of the automation (Muir, 1994;
Rempel et al., 1985);}
\item{ \textbf{faith}—the extent of belief that the automation will
be able to cope with future system states that it
may not yet have encountered (Madsen \& Gregor,
2000; Muir, 1994; Rempel et al., 1985)}
\end{enumerate}


\begin{comment}
\subsection{Levels of automation}
In \cite{Cummings04automationbias}, authors define a taxonomy of systems depending on their level of automation. According tho them, level of automation (LOA) can go from 1 (fully human without automation) to 10 (fully automated without humans). 

Since the European GDPR \cite{GDPR_2018} in its article 22 explicitly mentions the individual's right of not be subject on a decision based solely on automated processing, level of automation 6 would be the maximum allowed by the legislation and therefore, the maximum level of automation that could be considered as realistic nowadays.

In out experiment, we can test a variety of different scenarios, as described in table \ref{tab:levels_of_automation}.

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[H]
\centering
\begin{tabular}{@{}cc@{}}
\toprule
\textbf{\begin{tabular}[c]{@{}c@{}}Automation \\ Level\end{tabular}} & \textbf{Automation Description} \\ \midrule
2 & The computer offers a complete set of decision/action alternatives \\ \midrule
4 & suggest one alternative \\ \midrule
6 & allows the human a restricted time to veto before automatic execution \\ \bottomrule
\end{tabular}
\caption{Level of automation (LOAs) that can be used for our experiments}
\label{tab:levels_of_automation}
\end{table}

\subsection{Level of explanation}

\citet{javaidenhancing} measured trust and perception and their relation to the explanations on how the autonomous system took the decision.

They differentiate between \textit{static} and \textit{dynamic} explanations. Where the first are based upon (i) history and facts about the game, (ii) rules of the game and (iii) game-play tips; the latter provide insights into the \textit{evidences/knowledge based} robotic agent, showing \textit{how-type} and \textit{why-type} answers.

Authors of \cite{guidotti2018survey} provides a taxonomy of existing methods related to explainability. in their work, they made a classification of state of the art approaches by considering simultaneously the problem they are facing, the class of solutions proposed for the explanation, the kind of data analyzed and the type of predictor explained.

In their recent work, authors of \cite{beaudouin-hal-02507316} identified the characteristics to be considered when deciding the correct level of explanation in a given system, those where characterized between (i) Contextual factors, (ii) Technical solutions available, and (iii) Output format of the explanation.

Some authors have related the topic of Algorithmic explainability together with the notion of Algorithmic Accountability. In this direction, \cite{Bovens_2007} describes Algorithmic Accountability as \textit{A relationship between an actor and a forum, in which the actor has an obligation to explain and justify his or her conduct}. In his systematic literature review \cite{Wieringa_2020} categorizes existing techniques according to: (i) the actors level that can be individual, hierarchical, collective or corporate, (ii) the actor role, one between decision-maker, developers or users and (iii) aspect of the system is the actor responsible that for example could be testing or specification. 


\end{comment}


\subsection{Relation to algorithmic fairness}

The community of Algorithmic Fairness describes fairness as a concept that can be measured trough at least 21 different functions \cite{narayanan2018translation}. This measurement is often not aligned with the business goal of the system \cite{corbettdavies2017algorithmic} and mitigating certain metrics of fairness requires then to reduce overall system performance.

In this experiment, we wanted so simulate a similar scenario, where there is a decision support system (DSS) helping the player into deciding which is the next cell to be drilled.
%
This system has the particularity of being optimized for maximizing one variable: obtained oil, but ignores other variables. This is akin to many systems that try to optimize a \emph{proxy variable}.
%
For instance:

\begin{itemize}
    \item criminal recidivism prediction systems are trained with data on people who were \emph{convicted of a crime}, not people who \emph{committed a crime},
    \item emergency housing services prediction systems (Allegheny County) are trained with data on people who \emph{go to jail}, \emph{have multiple visits to emergency rooms}, or \emph{require in-patient mental health care}, not people who \emph{are homeless}.
\end{itemize}, 

Some algorithmic fairness issues can be traced to the usage of proxy variables.

==> Sections_OLD/3.Setting.tex <==
\section{Experimental Setup}
This section describes the scenario used to carry out the experiments\inote{the scenario or the tool? because if the important thing is the tool is not just an scenario}. After, we introduce the design of experiments used during the execution of the experiment and data collection phases.

\subsection{Scenario}
The implemented scenario consists on a web-based, online game designed with the objective of being easy to learn and easy to gain performance inside a given match. Also, it's designed to prevent this experience to fully generalize across multiple games, for that, the mechanics of the game do not change between different matches but the map varies between consecutive games.

The game has been inspired by the game \textit{Wildcat Wells}~\cite{Mason764} and consists on an board, composed by 32x32 cells and divided between dessert and forest cells. In each round, the player must select one cell in the board and the hidden value of that cell is then revealed and added to the score.

The game design has the particularity of including an environmental cost that the user will need to balance to obtain the best score. The cost of drilling the forest is significantly higher than drilling in the dessert. However, the intelligent system does not take into account the environmental cost, but only predicts the presence of oil. The oil model, that remains unknown to the user, is not correlated with the landscape model.

\subsection{Procedure}

The web interface is divided in two screens. The first is used to gather demographic information about the player and shows the historical ranking of players on the top right corner of the interface.
\begin{figure}[H] % picture
    \centering
    \includegraphics[width=0.7\textwidth]{Figures/game_ui1.png}
    \caption{Initial interface of the web application}.
\end{figure}

Between the demographic information, the following variables are gathered for each player:
\begin{enumerate*}
    \item Username
    \item Gender
    \item Age
    \item Country of residence
    \item Provenance (Student of our university or external user).
    \item Level of studies
    \item Background
\end{enumerate*}

The second screen, shown when the players selects the option "New game" shows the playing interface where the board is shown together with the accumulated income, environmental cost and aggregated score.

This landscape model is generated by using a Perlin noise \cite{Perlin_2002} generator. Using such noise, the obtained landscape looks more realistic than the random case. In the experiments, the environmental cost of drilling the forest is set to 20 whereas the cost of the dessert is zero.

\begin{figure}[H] % picture
    \centering
    \includegraphics[width=0.7\textwidth]{Figures/game_ui2b.png}
    \caption{Game interface showing the generated landscape}.
\end{figure}

Every time the player clicks a new cell on the board, the cell backgrounds changes and displays the obtained score for it. Also, the accumulated income (drilled oil) and environmental cost are increased.

The hidden oil model is generated using a simplified generator of Perlin noise \cite{Perlin_2002} that generates simple distributions, in most of the cases with one single global maximum. Values in the generated distribution range from 20 to 100.
\begin{figure}[H] % picture
    \centering
    \includegraphics[width=0.3\textwidth]{Figures/game_internal_model.png}
    \caption{Examples of generated hidden oil models. Yellow color corresponds to the areas with more oil.}
\end{figure}

A tutorial has been designed, where the basic mechanics of the game are explained. The presence of a tutorial elevates and equalized the initial knowledge users have when playing the first game.

\subsection{Achieving the game goal}
The game mechanics require then, to make an smart combination of exploration and exploitation to achieve the goal of obtaining the maximum score possible in a game. Each game consists of 15 rounds. The score is calculated as: \emph{Score} $=$ \emph{Income} $-$ \emph{Cost}, where the \emph{Income} comes from oil drilling, and the cost comes from drilling in the fores.
%
To achieve a high score, the player needs to balance the obtained score together with the environmental cost of drilling each of the selected cells. 


\subsection{Design of experiments}

\subsubsection{Map selection}
To reduce the variability driven by the random component during the map generation process, we conducted an initial experiment to select three maps to be used in the rest of the experimentation. To do so, we first randomly generated twenty-five different maps and manually selected ten different candidates from them.

After, we recruited a set of participants that played a game in one map randomly selected between the ten candidates, with an average of 10 games played per map.

We analyzed the behavorial traces from each map to select two maps where users where obtaining similar scores with a lower rate of initial plays direclty finding the global maximum (not-to-easy criteria). To these two, we included a third map selected between the ones that were identified to be easier according the the collected data. At the end of this process, the maps with ids $map_2$, $map\_3$ and $map\_7$ where selected.

\begin{figure}[H] % picture
    \centering
    \includegraphics[width=0.7\textwidth]{Figures/selected_maps.png}
    \caption{Oil and terrain plot of the three selected maps}.
\end{figure}

\subsubsection{Experimental units}
An experimental unit represents the set of conditions that a given player will face when participating in the experiment.

To remove the effects of the presentation order, participants played three games in a row.


\subsubsection{Experiment A}

\subsubsection{Experiment B}

\subsubsection{Experiment C}


==> Sections_OLD/4.1.ExperimentVariables.tex <==
\begin{enumerate}
    \item {Model accuracy
        \begin{enumerate}
            \item {Based on the number of probes allowed before the game begins
                \begin{enumerate}
                    \item Many probes $\rightarrow$ High performance
                    \item Few probes $\rightarrow$ Low performance
                \end{enumerate}
            }
        \end{enumerate}
    }
    \item {Whether to describe model accuracy (yes/no)
        \begin{enumerate}
            \item {Yes
                \begin{enumerate}
                    \item "The intelligent system is based on $X$ probes made in the same terrain, and on average over many games it can obtain a score of about $Y$ points per throw."
                \end{enumerate}
            }
        \end{enumerate}
    }
    \item {Model alignment with human goal (the machine does not know about costs)
        \begin{enumerate}
            \item High alignment: environmental cost is small or zero
            \item Low alignment: environmental cost is high
        \end{enumerate}
    }
    \item {How to display the recommendation
        \begin{enumerate}
            \item Automation level 2 - show an area
            \item Automation level 4 - show a point
        \end{enumerate}
    }
    \item {How to explain the recommendation
        \begin{enumerate}
            \item Provide explanation, e.g., display Voronoi diagram
            \item Do not provide explanation
        \end{enumerate}
    }
     \item {Reducing risk of loses vs increasing chance of earnings
        \begin{enumerate}
            \item Risk-driven: you lose points by doing something bad.
            \item Earnings-driven: you earn points by doing something good.
        \end{enumerate}
    }
\end{enumerate}

==> Sections_OLD/4.DoE.tex <==
\section{Design of (possible) experiments}
To define the set of possible experiments, we first differentiate between the control group and the experimental groups:

\begin{enumerate}
    \item \textbf{Control group:} We consider as control group a set of players that interacted with the game with no DSS activated. Therefore, their decisions and reactions to the game where not influenced by the machine predictions.
    \item {\textbf{Experimental groups:} The experimental groups are exposed to machine-based assistance. The set of variables considered for the experimental groups are summarized in the following section.
    }
\end{enumerate}     
\subsection{Explanatory or independent variables}
\input{Sections/4.1.ExperimentVariables}

\subsection{Dependent variables}
\begin{enumerate}
    \item {Trust in model 
    \begin{enumerate}
        \item Probability of the human of following a recommendation
        \item Self-assessment in exit poll as likert score
    \end{enumerate}
    
    }
    \item {Combined performance
    \begin{enumerate}
        \item Final score
        \item Time to completion
    \end{enumerate}
    }
\end{enumerate}





==> Sections_OLD/5.RQs.tex <==
\section{Key contributions with respect to the state of the art}

Between the key elements that differentiate our proposal from the existing state of the art, we consider the following elements as the most relevant ones:

\begin{itemize}
    \item \textbf{Accuracy (error) and alignment}.
    We can study the behavior of the system as a system that has both errors and biases or misalignment.
    %
    In our experiments, we have a target variable which is the benefit obtained by drilling oil and the decision support system is designed to optimize such variable.
    %
    In addition to it, there is also the \emph{Environmental Cost}, which is another variable that the user will care about (since it's used to calculate the final score) but it's not correlated with the initial one. This fact aims to reproduce a generally observed trend in productions systems, when they are designed to maximize profit for the company creating them (or some other proxy vaiable), but often tend to overlook other metrics or points of view that are of interest to the end-users.
    
    \item \textbf{Explanation of accuracy}. Our experiments will be based in an unique manner of explaining what's the expected performance of the decision support system's predictions. In this case, it will be expressed in the form of number of probes executed to train the current model. Practically, it is translated to the number of random points used to train the current model, and it will require that the user forms her own idea of what will this mean in terms of expected accuracy. 
    
\end{itemize}

\subsection{Research questions}
The design of experiments is driven by the initial research questions:
 \begin{quote}\emph{RQ. 1:Given a level of performance and alignment of a ML system, how do we maximize combined human-machine performance through transparency/awareness mechanisms}\end{quote}
 
 

\begin{comment}
    \begin{quote}\emph{RQ. 2: what transparency/explainability mechanisms yield best combined performance, under different contexts.}\end{quote}
    
    \begin{quote}\emph{RQ. 3: what experiences of working with a machine yield the best combined performance, under different contexts.}\end{quote}

\end{comment}



\subsection{Hypotheses (from literature)}
\begin{enumerate}
    \item Displaying model accuracy increases trust, \cite{yin_2019}
    \item Showing explanation increases trust, \cite{javaidenhancing}
    \item Automated decision-making leads to more accurate and/or fair outcomes \cite{Kleinberg_2017}
    \item When forecasters are deciding whether to use a human forecaster or a statistical
algorithm, they often choose the human forecaster, \cite{Diab_2011, Eastwood_2012}
    \item Seeing algorithms err makes people less confident in them, \cite{Dietvorst_2014}
    \item Overconfidence can lead to lower performance cause of the feeling of not need of assistance \cite{Arkes_1986}
\end{enumerate}

